Numerical Stochastic Perturbation Theory and the Gradient Flow

We study the Yang-Mills gradient flow using numerical stochastic perturbation theory. As an application of the method we consider the recently proposed gradient flow coupling in the Schr\"odinger functional for the pure SU(3) gauge theory.

==> sections/sec5.tex <==

\section{Conclusions \& outlook}

We studied the flow energy density $E$ in the SF at 3-loops
in perturbation theory for the pure SU(3) gauge theory. We reproduced the values
for $\mathcal{N}$ in~\cite{Fritzsch:2013je} and compared higher orders to 
MC results finding good agreement. Our study shows that a precise determination 
of $\overline{g}^2_{\rm GF}$ using  NSPT is feasible with moderate statistics. 
As a next step we plan to investigate the GF coupling in QCD. Larger lattice sizes
will be considered in order to extrapolate the matching coefficients to other schemes,
and the corresponding cutoff effects in the step-scaling function will be determined.


\section*{Acknowledgments}

The authors are grateful to M. L\"uscher, S. Sch\"afer, S. Sint, and R. Sommer for 
their valuable comments. We thank A. Ramos for kindly sharing material before 
publication, and F. Di Renzo and L. Scorzato for discussions. We also thank
M. Bruno, T. Harris, S. Lottini, and P. Vilaseca for kindly providing comments
on this manuscript. M.D.B. is supported by the Irish Research Council. 
D.H. acknowledges support by StrongNet. The code for MC simulations is 
based on the \texttt{MILC} package. ICHEC, TCHPC, and AuroraScience are 
acknowledged for the allocated resources. 

